FLAT: Fast, Lightweight and Accurate Method for Cardinality Estimation

Query optimizers rely on accurate cardinality estimation (CardEst) to produce good execution plans. The core problem of CardEst is how to model the rich joint distribution of attributes in an accurate and compact manner. Despite decades of research, existing methods either over simplify the models only using independent factorization which leads to inaccurate estimates, or over complicate them by lossless conditional factorization without any independent assumption which results in slow probability computation. In this paper, we propose FLAT, a CardEst method that is simultaneously fast in probability computation, lightweight in model size and accurate in estimation quality. The key idea of FLAT is a novel unsupervised graphical model, called FSPN. It utilizes both independent and conditional factorization to adaptively model different levels of attributes correlations, and thus dovetails their advantages. FLAT supports efficient online probability computation in near liner time on the underlying FSPN model, provides effective offline model construction and enables incremental model updates. It can estimate cardinality for both single table queries and multi table join queries. Extensive experimental study demonstrates the superiority of FLAT over existing CardEst methods on well known IMDB benchmarks: FLAT achieves 1 to 5 orders of magnitude better accuracy, 1 to 3 orders of magnitude faster probability computation speed and 1 to 2 orders of magnitude lower storage cost. We also integrate FLAT into Postgres to perform an end to end test. It improves the query execution time by 12.9% on the benchmark workload, which is very close to the optimal result 14.2% using the true cardinality.

==> flat.tex <==

% !TeX spellcheck = en_US

\section{Multi-Table C\lowercase{ard}E\lowercase{st}  Method}
\label{sec: flat}

In this section, we further discuss how to extend \FLAT algorithm onto multi-tables. 
We first describe the main framework, and then elaborate the two key techniques. 

\smallskip
\noindent{\underline{\textbf{Main Framework.}}}
To avoid ambiguity, in the following, we use printed letters, such as $T$, and calligraphic letters, such as $\mathcal{T}$, to represent a set of single tables and its corresponding full outer join table, respectively. Obviously, given a database $D$, all information of $D$ is contained in $\mathcal{D}$. To apply statistical models for \CE on $D$, one approach, such as~\cite{yang2020neurocard}, is to build a single model $M$ on $\mathcal{D}$ and uses it for any query.  It is easy and simple, but sacrifices efficiency. On one hand, the size of $\mathcal{D}$ grows exponentially in the number of tables in $D$, which in turn increases the model size. On the other hand, no matter how many tables are involved in a query, the entire, possibly large, model has to be used for probability computation.

Our \FLAT method tries another approach. It selects multiple subset of tables $D' \subseteq D$ and builds models $M'$ for each $\mathcal{D}'$. The final result is obtained by aggregating probabilities from multiple $M'$. This method is more efficient and adaptive. Moreover, unlike with existing work~\cite{hilprecht2019deepdb}, \FLAT is more general as it makes \emph{no} assumptions on the join types. In general, \FLAT has the following two procedures. 

\indent{\underline{\textit{1. Offline Construction}:}}
\FLAT first organizes all tables in $D$ as a tree $J$ based on their join relations.
Each node $T$ in $J$ is a table in $D$, and each edge $(T, P)$ in $J$ represents a join relation between table $T$ and $P$. The join is not restricted to the primary-foreign key join, but can be any operator, i.e., equal or unequal, between any pair of attributes. We can choose the join relations between tables from prior user knowledge of the database schema or find frequent joins from query workload~\cite{grahne2005fast}. It is also possible to maintain multiple trees to process different types of joins between tables. Meanwhile, we can make replicas of the same table to represent self-joins and loop-joins in the tree structure.

For each edge $(T, P)$ in $J$, we can either build the \FSPN on $T \fullouterjoin P$, the outer join table, or on each table individually. We apply a correlation-based testing method to decide which way is more appropriate. For each $(T, P)$ in $J$, we sample some records from $T \fullouterjoin P$, and examine the pairwise attribute correlation value between $T$ and $P$. If they are correlated on some attributes, it is better to learn on $T$ and $P$ together. Therefore, after examining all edges, for each node $T$ correlated with a neighbor $P$, we iteratively shrink $\{T, P\}$ to a single node. After that, $J$ is still a tree structure and each node $T$ in $J$ now represents a set of one or multiple tables. We construct a \FSPN $\F_{\T}$ on the outer join table $\mathcal{T}$ for each $T$ by using the method in Section~6. 

Figure~\ref{fig: flatexample} depicts a sample database with four tables and their join relations. 
The join relation between $T_{\A}$ and $T_\B$ on attribute $X$ is a many-to-many join. We build a join tree between them with three nodes $A, C$ and $D$. Since $T_{A}$ and $T_{B}$ are highly correlated, they are merged together into node $A$. We build a \FSPN on table $T_{\A} \fullouterjoin T_\B$ for node $A$.

\indent{\underline{\textit{2. Online Processing}:}}
Since tables in different nodes are weakly correlated, we can regard the probabilities of queries on different nodes to be mutually independent on the joined table. Therefore, the online probability computation phase follows a divide-and-conquer framework. For each query $Q$, we split it to multiple sub-queries on tables in each node $T$, computing probability of sub-query on $T$ by using the \FSPN $\F_{\T}$ and then aggregate them together to be the final result. Notice that, the sub-query probability computation and eventual aggregation are non-trivial tasks since the joint PDF on the join table is different from that on the single table. We elaborate the details of the sub-query probability computation and aggregation in the following Section~5.1 and~5.2, respectively. 


%\begin{figure}[t]
%	\scriptsize
%	\rule{\linewidth}{1pt}
%	\leftline{~~~~\textbf{Algorithm} \textsc{FLAT$(D, Q)$}}
%	\vspace{-1em}
%	\begin{algorithmic}[1]
%		\STATE \% offline processing
%		\STATE construct the joining tree $J$ based on $D$
%		\FOR{each $(T, P)$ in $J$}
%			\STATE obtain a sample of $T \fullouterjoin P$
%			\STATE compute the pairwise attribute correlation between $T$ and $P$
%		\ENDFOR
%		\WHILE{$|J|$ does not change}
%			\IF{there exists $(T, P)$ in $J$ and $T$ is highly correlated with $P$}
%				\STATE shrink nodes $T$ and $P$ into node $T$ in $J$
%			\ENDIF
%		\ENDWHILE
%		\STATE add columns $F_{\T, \N}$ by calling $\textsc{ScattCols}(J)$
%		\FOR{each node $T$ in $J$}
%			\STATE obtain the full outer join table $\mathcal{T}$ with all attributes $\mathcal{A}$
%			\FOR{each pair of joined tables $P, R$ in $T$}
%				\STATE add two columns $F_{\P, \R}$ and $F_{\R, \P}$ in $\mathcal{T}$
%			\ENDFOR
%			\STATE $\mathcal{F}_{T} \gets \textsc{Fspn-Struc}(\mathcal{A}, \emptyset, \mathcal{T}, \emptyset)$
%		\ENDFOR
%		\STATE \% online processing
%		\STATE get the size $|\mathcal{N}|$ of the full outer join table of nodes in $Q$
%		\STATE $p \gets 1$
%		\FOR{each node $T$ involved in $Q$}
%			\STATE set the constraint $C$ by Case~I
%			\STATE $Q[T] \gets Q[T] \textsc{ and } C$
%			\STATE get all joins $\{(P_{1}, R_{1}), (P_{2}, R_{2}), \dots, (P_{d}, R_{d} \}$ not in $Q_i$
%			\STATE $p_i \gets \textsc{Fspn-Infer}(\mathcal{F}_{\T}, R^{\Q[\T]})$ by Eq.~\eqref{eq: sqccorrect}
%			\STATE $p \gets p \cdot p_i$
%		\ENDFOR
%		\RETURN $|\mathcal{N}| \cdot p$
%	\end{algorithmic}
%	\smallskip
%	\rule{\linewidth}{0.7pt}
%	\leftline{~~~~\textbf{Procedure} \textsc{ScatterCols$(J)$}}
%	\vspace{-1em}
%	\begin{algorithmic}[1]
%		\STATE $k \gets 1$
%		\FOR{each node $T$ in $J$}
%			\STATE set $F_{\T, \{ \T \}} = 1$ for all records in $T$
%		\ENDFOR
%		\REPEAT
%			\FOR{each node $T$ in $J$}
%				\FOR{each $N$ rooted at $T$ that can be joined with table $S$}
%					\STATE obtain the path $P = (P_0, P_1, \dots, P_n)$ from $S$ to $T$
%					\STATE $F^{(0)} \gets F_{\S, \{ \S \}}$
%					\FOR{$i \gets 1$ to $n$}
%						\STATE compute $F^{(i)}$ by Eq.~\eqref{eq: recFstep}
%					\ENDFOR
%					\STATE add the column $F_{\T, \{ \N' \}}$ into table $\mathcal{T}$
%				\ENDFOR
%			\ENDFOR
%			\STATE $k \gets k + 1$
%		\UNTIL{$k$ cannot be enlarged}
%	\end{algorithmic}
%	\rule{\linewidth}{1pt}
%	\caption{Algorithm \FLAT for Cardinality Estimation.}
%	\label{fig: algflat}
%\end{figure}





\begin{figure*}
%\centering
\begin{flushleft}
\begin{minipage}{0.08\linewidth}
	\centering
	\textbf{Table $T_{\A}$} \\
	\begin{tabular}{|cc|}
	\hline
	$A_1$ & $A_2$ \\ \hline
	$b$ & 1 \\
	$a$ & 2 \\
	$c$ & 2 \\
	$b$ & 3 \\
	$c$ & 4 \\
	\hline
	\end{tabular}
\end{minipage}
\hspace{0.01\linewidth}
\begin{minipage}{0.12\linewidth}
	\centering
	\textbf{Table $T_{\B}$} \\
	\begin{tabular}{|ccc|}
		\hline
		$B_1$ & $B_2$ & $B_3$  \\ \hline
		0  & 0.32 & $M$ \\
		1  &  0.67 & $D$ \\
		4  & 0.79 & $Z$ \\
		1  &  0.39& $D$ \\
		2  & 0.41 & $B$ \\
		\hline
	\end{tabular}
\end{minipage}
\hspace{0.01\linewidth}
\begin{minipage}{0.2\linewidth}
	\centering
	\textbf{Table $T_{\C}$} \\
	\begin{tabular}{|cc|cc|}
		\hline
		$C_1$ & $C_2$  & $F_{\C, \{ \A \}}$ & $F_{\C, \{ \A, \D \}}$ \\ \hline
		$X$  & 0.26 & 0 & 0\\
		$P$  & 0.71 & 0 & 0\\
		$D$  & 0.88 & 2 & 4\\
		$N$  & 0.69 & 0 & 0\\
		$D$  & 0.27 & 2 & 4\\
		\hline
	\end{tabular}
\end{minipage}
\hspace{0.03\linewidth}
\begin{minipage}{0.2\linewidth}
	\centering
	\textbf{Table $T_{\D}$} \\
	\begin{tabular}{|cc|cc|}
		\hline
		$D_1$ & $D_2$  & $F_{\D, \{ \A \}}$ & $F_{\D, \{ \A, \C \}}$ \\ \hline
		$X$  & 60 & 0 & 0\\
		$D$  & 90 & 2 & 4\\
		$P$  & 77  & 0 & 0\\
		$D$  & 19 & 2 & 4\\
		$Y$  & 28 & 2 & 2\\
		\hline
	\end{tabular}
\end{minipage}
\begin{minipage}{0.3\linewidth}
	\centering
	\textbf{Joining Tree} \\
	\includegraphics[width = 0.8\linewidth]{figures/jointree.pdf}
\end{minipage}
\vspace{0.5em}

\hspace{0.05\linewidth}
\begin{minipage}{0.55\linewidth}
	\centering
	\textbf{Table $T_{\A} \fullouterjoin T_{\B}$} \\
	\begin{tabular}{|ccccc|cc|ccc|}
		\hline
		$A_1$ & $A_2$ & $B_1$ & $B_2$ & $B_3$ & $F_{\A, \B}$ & $F_{\B, \A}$
		& $F_{\A, \{ \C \}}$ & $F_{\A, \{ \D\}}$ & $F_{\A, \{ \C, \D \}}$
		\\ \hline
		\textsf{null} & \textsf{null} & 0 & 0.32 & $M$ & 0 & 1 & 0 & 0 & 0\\
		$b$ & 1 & 1 & 0.67 & $D$ & 2 & 1 & 2 & 2 & 4\\
		$b$ & 1 & 1 & 0.39 & $D$ & 2 & 1 & 2 & 2 & 4\\
		$a$ & 2 & 2 & 0.41 & $B$ & 1 & 2 & 0 & 0 & 0\\
		$c$ & 2 & 2 & 0.41 & $B$ & 1 & 2 & 0 & 0 & 0\\
		$b$ & 3 & \textsf{null} & \textsf{null} & \textsf{null} & 1 & 0 & 0 & 0 & 0\\
		$c$ & 4 & 4 & 0.79 & $Z$ & 1 & 1 & 0 & 0 & 0\\
		\hline
	\end{tabular}
\end{minipage}
\hspace{0.05\linewidth}
\begin{minipage}{0.3\linewidth}
	\centering
	\textbf{Example Queries} \\
	\begin{flushleft}
	$Q_1$: \textsf{select count(*) 
	from $T_\A, T_\B$ \\
	\underline{where $T_{\A}.A_1 = b$ and $T_{\B}.B_2 >= 0.45$} } \\	
	$Q_2$: \textsf{select count(*) 
		from $T_\B$ \\
	\underline{where $T_{\B}.B_2 >= 0.2$ and $T_{\B}.B_2 <= 0.5$}} \\
	$Q_3$: \textsf{select count(*) 
	from $T_\B, T_\C, T_\D$ \\
	where $T_{\B}.B_3 = T_{\C}.C_1$ and $T_{\B}.B_3 = T_{\C}.D_1$ and $T_{\B}.B_2  >  0.35$
		and $T_{\C}.C_2  <  0.3$ and $T_{\D}.D_2 > 75$}
	\end{flushleft}
\end{minipage}

\end{flushleft}
\caption{Example databases and join queries.}
\label{fig: flatexample}
\end{figure*}



\subsection{Sub-Query Probability Computation}

Given a query $Q$ on tables in node $T$, let $\mathcal{P}$ denote the join table specified by $Q$.
Notice that, $\mathcal{P}$ may differ from $\mathcal{T}$---the full outer join table of all tables in $T$---due to two reasons: First, $Q$ may use different join, such as inner join, between tables in $T$.
Second, $Q$ may only touch a subset of tables in $T$. For example, the query $Q_2$ in Figure~\ref{fig: flatexample} is only on table $T_{\B}$ in node $A$. The joint PDF of attributes in table $\mathcal{P}$ and $\mathcal{T}$ are also different. Therefore, to obtain the exact cardinality of $Q$, the computed probability needs to be corrected a bit. We elaborate the methods in this subsection.

For any pair of joined tables $A, B$ in $T$, each record in $A$ can join with multiple records in $B$ and vice versa. We add two additional attributes $S_{\A, \B}$ and $S_{\B, \A}$ in $\mathcal{T}$. $S_{\A, \B}$ indicates how many records in $B$ can join with this record in $A$ and vice versa. $S_{\A, \B} = 0$ indicates a record in $A$ has no match in $B$. Obviously, for a primary-foreign key join from $A$ to $B$, $S_{\A, \B}$ can only be $0$ or $1$. For example in Figure~\ref{fig: flatexample}, we add two columns $S_{\A, \B}$ and $S_{\B, \A}$ in the table $T_{\A} \fullouterjoin T_{\B}$. The last tuple $(2, 0.41, B)$ in $T_{\B}$ can join with two records in $T_{\A}$, so we have $S_{\B, \A} = 2$. 
We call such $S_{\A, \B}$ the \emph{scatter coefficient}. These columns are built together with other attributes in constructing the \FSPN $\F_{\T}$, so we can also specify predicates on them to obtain the corresponding probability. With their assistance, the probability $\Pr_{\mathcal{T}}(Q)$ can be corrected as follows:

\underline{\textit{Case~I (Query with Different Join)}}: 
For any pair of joined tables $A$ and $B$ in $T$, if query $Q$ is on the inner-join table $A \! \bowtie \! B$, in comparison with $A \fullouterjoin B$, we just need to remove all records in $A$ or $B$ that have no matches in the other table, i.e., $S_{\A, \B} = 0$ or $S_{\B, \A} = 0$, from $A \fullouterjoin B$. Thus, we can add the constraint $S_{\A, \B} > 0$ and $S_{\B, \A} > 0$ into $Q$ to be $Q'$. Similarly, if $Q$ is on the left-join table $A \leftouterjoin B$ or right join table $B \rightouterjoin A$, we only add $S_{\A, \B} > 0$ or $S_{\B, \A} > 0$ to $Q$, respectively. Obviously, we have $\Card(\mathcal{P}, Q) =  \Pr\nolimits_{\mathcal{T}} (Q') \cdot |\mathcal{T}|$. For example, in Figure~\ref{fig: flatexample}, for the query $Q_1$ on table $T_{\A} \! \bowtie \! T_{\B}$, we have $\Pr_{\mathcal{T}} (Q_1 \textsc{ and } S_{\A, \B} > 0 \textsc{ and } S_{\B, \A} > 0) = 1/7$, so the estimated cardinality is $1$. 

\underline{\textit{Case~II (Query with Subset of Tables)}}: 
As each record in $\mathcal{P}$ has been scattered multiple times in $\mathcal{T}$, we need to correct the probability by removing this effect. Let $U = \{(A_{1}, B_{1}), (A_{2}, B_{2}), \dots, (A_{n}, B_{n}) \}$ denote all join relations in $\mathcal{T}$ but not touched in $Q$ and $S_{\U}$ be its corresponding scattering columns. Let $s = (s_1, s_2, \dots, s_n)$ where $s_i \in \mathbb{N}$ and $S_{\A_{i}, \B_{i}} = s_i$ for all $1 \leq i \leq n$ denote an assignment of values to all scattering columns in $S_\U$. We have
\begin{equation}
\small
\label{eq: tcqcomplex}
\Pr'\nolimits_{\mathcal{T}} (Q) = \sum_{s} 
\frac{\Pr_{\mathcal{T}}(Q \textsc{ and } S_\U = s )}
{\text{den}(s)},
\end{equation}
where $\text{den}(s) = \prod_{i=1}^{n} \max\{s_i, 1\}$ since we also need to count the records satisfying $Q$ but have no matches in $\mathcal{T}$, i.e., $s_i = 0$ for some $A_{i}, B_{i}$. Then, we must have
$\Card(\mathcal{P}, Q) =  \Pr'\nolimits_{\mathcal{T}} (Q) \cdot |\mathcal{T}|$.
Take the query $Q_2$ in Figure~\ref{fig: flatexample} as an example. Since $Q_2$ is only on table $T_{\B}$, we have $U = \{(T_\B, T_\A)$ and obtain $\Pr'_{\mathcal{T}} (Q_2) = 2/7 + (2/7)/2 = 3/7$, so 
the estimated cardinality is $3$.

If Case~1 and Case~2 both exist, we first obtain the query $Q'$ by adding constraints on the scattering columns, and then correct the probability on $Q'$ to$\Pr'_{\mathcal{T}}(Q')$. Certainly, we have $\Card(\mathcal{P}, Q) =  \Pr'\nolimits_{\mathcal{T}} (Q') \cdot |\mathcal{T}|$.

\smallskip
\noindent{\underline{\textbf{Fast Computation of $\Pr'\nolimits_{\mathcal{T}} (Q')$}:}}
It is worth mentioning that the probability $\Pr'\nolimits_{\mathcal{T}} (Q')$ could be computed in a fast way on \FSPN without needing to access each assignment as in Eq~\eqref{eq: tcqcomplex}. Let $S$ and $A$ denote all scatter coefficients columns and attribute columns in $\mathcal{T}$, respectively. Let $S_1$ be all scattering columns added to $Q$ by Case~1. We denote  $S_1 > 0$ to indicate that each column in $S_1$ is larger than $0$. Let $S_2$ denote all scattering columns to be explored by Case~2. 

In the \FSPN $\F_{T}$, we first use a \textsf{factorize} node to losslessly split $\Pr_{\mathcal{T}}(S, A)$ to $\Pr_{\mathcal{T}}(A)$ on the left child $X$ and $\Pr_{\mathcal{T}}(S | A)$ on the right child $Y$. By the property of \FSPNend, each leaf node $L$ of $Y$ models a joint PDF on all $S$ and the conditions on $Q$ and $S$ must be independent on $Y$. Then, we must have
\begin{equation}
\small
\label{eq: tcqcomplexfast}
\Pr'\nolimits_{\mathcal{T}} (Q') = \sum_{\L}  \left( Pr_{\mathcal{T}_\X}(Q) \cdot 
\sum_{s} \frac{\Pr_{\mathcal{T}_\L}(S_1 > 0 \textsc{ and } S_2 = s )}
{\text{den}(s)} \right).
\end{equation}
The left probability $Pr_{\mathcal{T}_\X}(Q)$ is only on attributes $A$ and could be computed in the same way as in Section~4. For the remaining right part\footnote{We omit the weight for simplicity.}, 
when $S_1$ and $S_2$ are given, it is a \emph{fixed} expectation value of $1 / \text{den}(s)$ on all points in $S$ such that $S_1 > 0$. Therefore, we can pre-compute and store it offline. After that, we can discard the PDF on $S$ maintained in each leaf $L$. The space cost to store these values on each leaf node is $O(4^{|S|})$, which is affordable since $|S|$ is often small. Moreover, it is more economical than the space cost to maintain the multi-dimensional PDF of $S$.


\subsection{Sub-Query Probability Aggregation}

Given a query $Q$, let $P = \{T_{1}, T_{2}, \dots, T_{d} \}$ denote all nodes in $J$ touched by $Q$.
For all $1 \leq i \leq d$, let $Q_i$ be the sub-query on tables in node $T_i$. By the method in Section~5.1, we could obtain the probability $\Pr'_{\mathcal{T}_i}(Q'_i)$ such that $\Pr'_{\mathcal{T}_i}(Q'_i) \cdot |\mathcal{T}_i|$ is the estimated cardinality of $Q_i$. 
By our assumption, the probability on different nodes are mutually independent on $\mathcal{P}$---the full table joining $\mathcal{T}_i$ for all nodes in $P$.


After we process the sub-query $Q_i = Q[T_{i}]$ on each node $T_{i}$ and obtain the probability $\Pr_{\mathcal{T}_{i}}(Q_i)$, we need to combine them together to be the final result. 
By our assumption, the probabilities on different nodes are mutually independent, so we have 
\begin{equation}
\Pr\nolimits_{\mathcal{N}}(Q) = \prod_{i = 1}^{n} \Pr\nolimits_{\mathcal{N}}(Q_{i}).
\end{equation}
However, by now, we only have the probability $\Pr_{\mathcal{T}_{i}}(Q_i)$ following Section~4.2, which differs with $\Pr_{\mathcal{N}}(Q[T_{i}])$ since records in $\mathcal{T}_{i}$ would be scattered after joining tables in different nodes. Therefore, we also need to expand \textbf{ *** expand what? ***} to correct the scattering effects.

Similarly, we also assume there exists a column $F_{T_{i}, N}$ in table $\mathcal{T}_i$ indicating the scattering coefficient of each record in $\mathcal{T}_{i}$ to the outer join table $\mathcal{N}$. From Eq.~\eqref{eq: tcqcomplex}, we have 
\begin{equation}
\small
\label{eq: sqccorrect}
\begin{split}
& \Pr\nolimits_{\mathcal{N}}(Q_i) = \\
& \frac{\sum\limits_{f, f_1, f_2, \dots, f_d}  \!\!\!\!\!\!\!\!
	\frac{\Pr_{\mathcal{T}}(Q_i \textsc{ and }  F_{T_{i}, N} = f \textsc{ and } F_{\P_{1}, \R_{1}} = f_1 \textsc{ and } \dots F_{\P_{d}, \R_{d}} = f_{d} ) \cdot \max\{f, 1\}}
	{\prod_{j=1}^{d} \max \{f_j, 1\}}
}
{\sum_{f} \Pr\nolimits_{\mathcal{T}_{i}}(F_{T_{i}, N} = f) \cdot \max\{f, 1\}}.
\end{split}
\end{equation}
Here $f_1, f_2, \dots, f_d$ are used to correct the scattering effects of tables not touched by $Q_i$ in $T_i$ and $f$ downscales the scattering effects of expanding $\mathcal{T}_i$ to $\mathcal{N}$. We can learn all columns $F_{T_{i}, N}$ with other attributes in the \FSPN together and apply the method in Section~4.2 to efficiently compute Eq.~\eqref{eq: sqccorrect}. 

Finally, we multiply all probabilities $\Pr_{\mathcal{N}}(Q_i)$ together and obtain the cardinality of $Q$ as
\begin{equation}
\Card(\mathcal{N}, Q) = |\mathcal{N}| \cdot \Pr\nolimits_{\mathcal{N}}(Q).
\end{equation}
The size $\mathcal{N}$ could also be estimated by using the sampling method in~\cite{}. Remarkably, if the join types across two nodes $T_i$ and $T_j$ are not outer joins, as $F_{T_i, \{ T_j\}}$ is also learned in the \FSPN of $T_i$, we can add the constraint to $Q_i$ in a similar way as Case~I in Section~4.2.

For example, consider the query $Q_3$ in Figure~\ref{fig: flatexample} which is across the three nodes $A, C$ and $D$. First, for the sub-query $Q_3[A]$ on node $A$, we need to use the column $F_{\B, \A}$ to downscale the scattering effects in $T_{\A} \fullouterjoin T_\B$ to $T_{\B}$ and the column $F_{\A, \{\C \D\} }$ to expand the scattering effects in from $T_{\A} \fullouterjoin T_\B$ to $T_{\A} \fullouterjoin T_\B \fullouterjoin T_\C \fullouterjoin T_\D$. By Eq.~\eqref{eq: sqccorrect}, we have $\Pr(Q_{3}[A]) = 1* 4 / (4 + 4)= 1/2$. In the same way, we also have $\Pr(Q_{3}[C]) = 1/2$ and $\Pr(Q_{3}[D]) = 1/2$. The final estimated cardinality is $8 * (1/8) = 1$.


\smallskip
\noindent{\underline{\textbf{Scatter Coefficients Columns Construction.}}}
By now, the only remaining thing is to construct the scatter coefficients columns $F_{\T, \{\N\} }$ for each node $T$ and each possible $N$. $N$ can be regarded as a 
sub-tree expanding from the root $T$. Given the structure of $N$, we can compute 
$F_{\T, \{\N\}}$ in the following bottom-up manner:

1. For each leaf node $L$ in the sub-tree $N$, set the column $F_{\L} = 1$ for all records.

2. For each non-leaf node $O$ in $N$, for each record $t$, we have 
\begin{equation}
\label{eq: recF}
F_{O}[t] = \prod_{H \in \text{Children}(O)} \sum\nolimits_{t' \in H \text{ joining } t} F_{H}[t'].
\end{equation}
Finally, we obtain $F_{\T, \{\N \}} = F_{\T}$. Based on this, we propose a \emph{dynamic programming} method \textsc{ScatterCols} called in line~9 of the \textsc{FLAT} algorithm to construct $F_{\T, \{\N \}}$. We list the detailed steps in Fig.~\ref{fig: algflat}. The rules are as follows:\\
\indent \underline{\textit{Rule I} (lines~1--3)}: for all node $T$ in $J$, we set $F_{\T, \{\T\}}$ to be $1$ for all records. Set $k = 1$. 

\indent \underline{\textit{Rule II} (lines~4--13)}: from $k = 1$, for each node $T$ and each $N$ rooted at $T$ containing $k$ nodes, for each node $S$ that can join with $N$, let $N' = N \cup \{S\}$, we try to obtain $F_{\T, \{\N' \}}$. Note that, since $N$ is a tree structure, there exists only one path $P = (P_0, P_1, \dots, P_n)$ from $S$ to $T$ where $P_0 = S$ and $P_n = T$.
Let $F^{(0)} = F_{\S, \{\S \}}$. For all $1 \leq i \leq n$, let
\begin{equation}
\label{eq: recFstep}
F^{(i)}[t] = F_{P_i, \{B_i \! \}} [t] \cdot \!\!\!\! \sum\limits_{t' \in P_{i-1} \text{ joining } t} \!\!\!\!\!\!\!\!  F^{(i - 1)}[t'], 
\end{equation}
where $B_i$ denote all tables joining with $P_i$ in $N$ but not on the path $P$. 
Since $|B_i| < k$, the columns $F_{P_i, \! \{B_i\!\}}$ have already been computed and stored in the table $\mathcal{P}_i$. By Eq.~\eqref{eq: recF}, we have $F_{\T, \! \{\N' \! \} } = F^{(n)}$. After scanning all $N$ with $|N| = k$, we increase $k$ by $1$.

Note that, the \textsc{ScatterCols} procedure is efficient since the node size $|J|$ of the 
coarsened tree $J$ is small. Meanwhile, it is easy to implement in parallel across different nodes and in scanning tables for computing Eq.~\eqref{eq: recFstep}.

We continue with the example in Figure~\ref{fig: flatexample}.
For node $A$, we first compute the columns $F_{\A, \{\C\}}$ and $F_{\A, \{\D\}}$ by scanning elements in $T_{\C}$ and $T_{\D}$, respectively. 
Then, we expand from $F_{\A, \{\C\}}$ to $F_{\A, \{\C \D \}}$. At this time, we have $P_0 = D$ and $P_1 = A$. For $i = 1$, $B_1 = C$, we obtain $F_{\A, \{\C \D \}} = F^{(1)}$ by Eq.~\eqref{eq: recFstep}. $F_{\A, \{\C \D \}}$ represents the scattering coefficients of records in node $A$ in the star-join from $A$ to node $C$ and $D$. The columns 
$F_{\C, \{\A\}}$ and $F_{\C, \{\A \D\}}$ in node $C$ and columns 
$F_{\D, \{\A\}}$ and $F_{\D, \{\A \C\}}$ in node $D$ are computed in a similar way. However, $F_{\C, \{\A \D\}}$ represents the scattering coefficients of records in node $C$ in the chain-join from $C$ to node $A$ to $D$. Note that, the values in the column $F_{\C, \{\A \D\}}$ and 
$F_{\D, \{\A \C\}}$ are different. 



==> struc.tex <==

% !TeX spellcheck = en_US

\section{\FSPN Structure Construction}
\label{sec: struc}

By now, the only remaining task is to present how to construct a \FSPN structure from data. 
Unlike with \textsf{BN}, structure construction of \FSPN is much easier. We first present the general idea, and then give the detailed algorithm.

\smallskip
\noindent{\underline{\textbf{General Idea.}}}
We present the general process for constructing \FSPN on a table $T$ with attributes $A$ in Figure~\ref{fig: fspnstruc}. 
It works in a top-down manner to dentify different operations to decompose the joint PDF. 
First, we test if there exists a set of high correlated attributes $H$ in $A$. If so, let $L = A - H$. We add a \textsf{factorize} node to decompose the joint PDF as $\Pr_{\T}(L)$ and $\Pr_{\T}(H | L)$.
For $\Pr_{\T}(H | L)$, we split all records in terms of the condition 


The 




\begin{figure}
	\includegraphics[width = \columnwidth]{figures/fspnemp-2.pdf}
	\caption{\FSPN Structure Construction Process.}
	\label{fig: fspnstruc}
	\vspace{-1em}
\end{figure}

Unlike learning the structure of a \textsf{BN}, building a \FSPN from data is much easier.
The algorithm \textsc{Fspn-Struc} for constructing an \FSPN structure is described in detail in Figure~\ref{fig: algfspnstru}. Its general idea is illustrated in the middle of Figure~\ref{fig: fspnexample}.
\textsc{Fspn-Struc}  works in a top-down manner to identify different operations to decompose the joint PDF. For each node $N$, it recursively generates its descendants. The inputs of 
\textsc{Fspn-Struc} on node $N$ include the scope of attributes $A_\N$, the condition of attributes $C_\N$, the context of records $T_\N$ and an attribute subset $I_\N \subseteq C_\N$ recording attributes in $C_\N$ independent of $A_\N$. We can  obtain the \FSPN $\F$ by directly calling $\textsc{Fspn-Struc}(A, \emptyset, T, \emptyset)$. 
Generally, \textsc{Fspn-Struc} follows the following steps.

\smallskip
1) \underline{\textit{Leaf Node Processing (lines 1--8)}}: 
At first, we examine whether $N$ should be a leaf node. 
If $C_{\N} = \emptyset$, $|A_\N| = 1$ or $C_{\N} \neq \emptyset$, $I_\N = C_\N$, $N$ is a \textsf{prob-node} and \textsf{cond-node} leaf, respectively. We call the procedure \textsc{PDFModel} to obtain (an estimate of) \textbf{ *** this used to be "model". But at least in my opinion "model" is not the same as the estimate/approximation obtained by using a model ***} $\Pr_{\T_{\N}}(A_\N)$. \textsc{PDFModel} may be implemented using off-the-shelf tools~\cite{poosala1997selectivity,rasmussen2000infinite} to estimate univariate and multivariate PDFs for highly correlated random variables. In our implementation, we choose the  histograms~\cite{poosala1997selectivity} and parametric Gaussian mixture functions~\cite{rasmussen2000infinite} to model categorical and continuous attributes, respectively. 

If $N$ is not a leaf node, we decide its operation $O_{\N}$.
The \textsc{Cor} procedure estimates correlation between two attributes using e.g. RDC~\cite{lopez2013randomized}. Two pre-defined thresholds $\tau_{h}$ and $\tau_{l}$ are used to filter highly correlated and independent relations, respectively. \textbf{ *** again, we might want to be more precise w.r.t the whole correlation/independence terminology ***}

\smallskip
2) \underline{\textit{\textsf{Prob-Node} Processing (lines 9--25)}}: 
If $N$ is a \textsf{prob-node}, we compute pairwise correlations between all attributes in $A_\N$ and encode the results in two undirected graphs $G_h$ and $G_l$. Vertices of $G_h$ and $G_l$ are all attributes in $A_\N$. Two attributes $f, g$ are connected in $G_h$ and $G_l$ if $\textsc{Cor}(f, g) \geq \tau_{h}$ and $\textsc{Cor}(f, g) \geq \tau_{l}$, respectively. 
Obviously, if $G_h$ has some edges, each connected component stands for a set of highly correlated attributes. At this time, we can use the \textsf{factorize} operation on node $N$. We pick $H$, the 
largest connected component in $G_{h}$, add two children of node $N$ on $A_\N - H$ and $H$ accordingly, and recursively call \textsc{Fspn-Struc} on them.

If $G_h$ has no edge, we further check $G_l$. If $G_l$ is not connected, let $A'_1, A'_2, \dots, A'_m$ denote all of its connected components. Certainly, attributes in different $A'_j$ are mutually independent, so we use the \textsf{product} operation on node $N$. For each $j$, we project $T_\N$ as $T_\N[A'_j]$ and continue processing the children on $A'_j$,

Otherwise when $G_l$ is connected, we could use the \textsf{sum} operation to split records in $T_\N$ to create contextual independency \textbf{*** create sets on which independence holds? ***}. According to~\cite{} \textbf{*** Reference? ***}, we can apply a clustering method \textsc{Cluster}, such as $k$-means~\cite{krishna1999genetic}, to split $T_\N$ to $T_1, T_2, \dots, T_n$. Intuitively, records in the same cluster are  similar so the corresponding PDF becomes simpler and smoother. As a result, attributes are more likely to be independent. We then call \textsc{Fspn-Struc} on each child $T_i$ with weight $w_i = {|T_i|}/{|T_\N|}$.

\smallskip
3) \underline{\textit{\textsf{Cond-Node} Processing (lines 26--34)}}: 
If $N$ is a \textsf{cond-node}, we compute pairwise correlations across all attributes in $A_\N$ and $C_\N - I_\N$. Let $c \in C_\N - I_\N$ be an attribute satisfying $\max_{s \in A_\N} \textsc{Cor}(s, c) < \tau_{l}$. $c$ is already independent of $A_{\N}$, so we add it into $I_{\N}$ and do not split it further. This is because our splitting operation gradually decreases the correlations between $A_\N$ and $C_{\N}$, $c$ is less likely to be dependent of $A_{\N}$ in the descendants of node $N$. After that, if $I_\N = C_\N$, we can further call \textsc{Fspn-Struc} to process this leaf node. Otherwise, we use the \textsf{sum} operation to further split records in $T_\N$ to create contextual conditional independency. The splitting task is fulfilled by the \textsc{GridSplit} method, which returns $T_1, T_2, \dots, T_n$ according to attributes $C_\N - I_\N$. After that, we further call \textsc{Fspn-Struc} on each child $T_i$ with weight $w_i = {|T_i|}/{|T_\N|}$.

Next we describe the details of the the \textsc{GridSplit} procedure. Notice that, for convenience of the inference process, it is required that the attribute values in each cluster $T_i$ must stay in a grid. To achieve this, \textsc{GridSplit} method applies a heuristic 2-way partition. Each time, it chooses an attribute $X \in C_\N - I_\N$ and a point $x$ in the value interval of $X$ to split $T_{\N}$ into two parts. For example, in node $N_3$ in Figure~\ref{fig: fspnexample}, we choose the attribute TP and value $60^\circ\text{F}$ to split all records. Generally, $X$ and $x$ are chosen according to the following metric. For each attributes $X \in C_\N - I_\N$, let $K_{X}$ be a pre-defined hyper-parameter.
We choose $K_{X} - 1$ points $x_i$ to evenly divide the value interval of $X$. For each $x_i$, we can try to split $T_{\N}$ into two parts. Let $m = \max_{s, c} \textsc{Cor}(s, c)$ where $s \in A_{\N}, c \in C_{\N} - I_{\N}$ denote the maximum correlation values across attributes in $A_\N$ and $C_\N - I_\N$.
Let $m_{i}^{\L}$ and $m_{i}^{\R}$ denote the value $m$ of the left and right cluster generated by $x_i$, respectively. We can use $\max(m_{i}^{\L}, m_{i}^{\R})$ to represent the division quality of point $x_i$. Obviously, the less value is \textbf{*** ? the fewer values there are ? ***}, the more likely that attributes in $C_\N - I_\N$ are independent of $A_\N$ in each cluster. We pick the attribute $X$ and the point $x_i$ which minimizes this quality value to divide the context of records $T_{\N}$. 

Notice that, the \textsc{Fspn-struc} algorithm resembles more of a general framework than a concrete algorithm. We can easily develop and integrate new correlation metrics, clustering and splitting methods depending on different requirements and circumstances.



